ELMI: Interactive and Intelligent Sign Language Translation of Lyrics for Song Signing

d/Deaf and hearing song-signers have become prevalent across video-sharing platforms, but translating songs into sign language remains cumbersome and inaccessible. Our formative study revealed the challenges song-signers face, including semantic, syntactic, expressive, and rhythmic considerations in translations. We present ELMI, an accessible song-signing tool that assists in translating lyrics into sign language. ELMI enables users to edit glosses line-by-line, with real-time synced lyric and music video snippets. Users can also chat with a large language model-driven AI to discuss meaning, glossing, emoting, and timing. Through an exploratory study with 13 song-signers, we examined how ELMI facilitates their workflows and how song-signers leverage and receive an LLM-driven chat for translation. Participants successfully adopted ELMI to song-signing, with active discussions throughout. They also reported improved confidence and independence in their translations, finding ELMI encouraging, constructive, and informative. We discuss research and design implications for accessible and culturally sensitive song-signing translation tools.

==> tables/table-butter-translation.tex <==
\def\lyriccolumnwidth{0.20\textwidth}
\def\examplecolumnwidth{0.40\textwidth}


\begin{table}[]
\sffamily
\small
	\def\arraystretch{1.1}\setlength{\tabcolsep}{0.25em}
		    \centering
\caption{Summary of participants' translation of \assignedsong{}, including the word count of gloss lines and the average of pairwise overlap coefficient across participants' gloss words for the same line. 0\% of average overlap means that all glosses from participants include distinct words.}
\Description{This table summarizes participants' translations of the song "BTS-Butter," showing the word count of gloss lines and the average pairwise overlap coefficient across participants' gloss words for each lyric line. The table includes columns for each lyric line, the original English lyric, the language (ASL or PSE), an example gloss from participants, the minimum, maximum, mean, and standard deviation of the word count in glosses, and the average overlap percentage. The overlap percentage indicates how much participants' glosses for the same line use similar words. Each row provides detailed data for specific lyric lines.}
\label{tab:results:translation:all}
\begin{tabular}{|c!{\color{gray}\vrule}m{\lyriccolumnwidth}!{\color{gray}\vrule}c!{\color{lightgray}\vrule}m{\examplecolumnwidth}!{\color{lightgray}\vrule}cccc!{\color{lightgray}\vrule}c|}
\hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                & \cellcolor[HTML]{EFEFEF}                                 & \cellcolor[HTML]{EFEFEF}                                & \cellcolor[HTML]{EFEFEF}                                         & \multicolumn{4}{c!{\color{lightgray}\vrule}}{\cellcolor[HTML]{EFEFEF}\textbf{Gloss word count}}                                                                                  & \cellcolor[HTML]{EFEFEF}                                            \\
\rowcolor[HTML]{EFEFEF} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Line}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Lyric}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Lang}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Example gloss}} & {\color[HTML]{333333} \textbf{Min}} & {\color[HTML]{333333} \textbf{Max}} & {\color[HTML]{333333} \textbf{Mean}} & {\color[HTML]{333333} \textbf{Std}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\parbox[t]{0.07\textwidth}{\centering \textbf{Average Overlap}}} \\
\hline
                                                        &                                                          & ASL                                                     &                                                   ME SAME-AS BUTTER SMOOTH (\p{10})               & 2                                   & 5                                   & 3.50                                 & 1.22                                & 67.33\%                                                              \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{1}                                     & \multirow{-2}{*}{Smooth like butter}                     & PSE                                                     &                      SMOOTH LIKE BUTTER (\p{6}, \p{8}, \p{11})                                            & 3                                   & 5                                   & 3.80                                 & 1.10                                & 62.00\%                                                              \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &                                       PERSON DANGEROUS DISGUISE (\p{3})                           & 2                                   & 3                                   & 2.83                                 & 0.41                                & 0.00\%                                                               \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{2}                                     & \multirow{-2}{*}{\parbox[t]{\lyriccolumnwidth}{Like a criminal\newline{}undercover}}             & PSE                                                     &                   LIKE SECRET THIEF (\p{7})                                               & 3                                   & 5                                   & 3.60                                 & 0.89                                & 32.50\%                                                             \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &                 GUN [LCL``shoot"] (\p{2})                                                 & 1                                   & 4                                   & 2.83                                 & 1.17                                & 11.11\%                                                              \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{3}                                     & \multirow{-2}{*}{Gon' pop like trouble}                  & PSE                                                     &                  APPEAR LIKE TROUBLE (\p{8}, \p{11})                                                & 3                                   & 4                                   & 3.20                                 & 0.45                                & 50.00\%                                                              \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &               PENETRATE HEART HEART [CL ``pump"] (\p{10})                                                   & 2                                   & 5                                   & 3.17                                 & 1.17                                & 53.33\%                                                             \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{4}                                     & \multirow{-2}{*}{\parbox[t]{\lyriccolumnwidth}{Breakin' into your heart\newline{}like that}}     & PSE                                                     &                                         ME ENTER YOUR HEART (\p{6})                         & 3                                   & 5                                   & 4.40                                 & 0.89                                & 22.33\%                                                             \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &            [CL:1 ``person wearing sunglasses, looking cool"] [HEAD-tilt ``same as music video"] (\p{2})                                                      & 0                                   & 4                                   & 2.83                                 & 1.17                                & 22.22\%                                                             \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{5}                                     & \multirow{-2}{*}{Cool shade stunner}                     & PSE                                                     &               COOL SHADE AWESOME PERSON (\p{7})                                                   & 1                                   & 4                                   & 3.00                                 & 1.22                                & 9.17\%                                                              \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &               [HEAD-nod] THANK MOTHER (\p{2})                                                   & 2                                   & 6                                   & 3.50                                 & 1.38                                & 21.67\%                                                              \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{6}                                     & \multirow{-2}{*}{\parbox[t]{\lyriccolumnwidth}{Yeah, I owe it all\newline{}to my mother}}        & PSE                                                     &                                     ME OWE MOM EVERYTHING (\p{8})                             & 3                                   & 7                                   & 5.40                                 & 1.82                                & 27.86\%                                                             \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &                 SUNSHINE [CL:5 ``coming from me "] (\p{10})                                                 & 1                                   & 4                                   & 2.67                                 & 1.03                                & 55.56\%                                                              \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{7}                                     & \multirow{-2}{*}{Hot like summer}                        & PSE                                                     &               HOT LIKE SUMMER (\p{6}, \p{8})                                                   & 3                                   & 5                                   & 4.00                                 & 1.00                                & 79.83\%                                                             \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &                    YOU SWEAT YES (\p{12})                                              & 2                                   & 5                                   & 3.67                                 & 1.21                                & 46.11\%                                                             \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{8}                                     & \multirow{-2}{*}{\parbox[t]{\lyriccolumnwidth}{Yeah, I'm makin' you\newline{}sweat like that}}   & PSE                                                     &                                     ME CAUSE YOU SWEAT (\p{4}, \p{6}, \p{8})                             & 2                                   & 8                                   & 4.60                                 & 2.79                                & 40.36\%                                                             \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &                    RELAX ENJOY (\p{2})                                              & 1                                   & 4                                   & 2.00                                 & 1.10                                & 6.67\%                                                              \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{9}                                     & \multirow{-2}{*}{Break it down}                          & PSE                                                     &                  DANCE (\p{8})                                                & 1                                   & 3                                   & 1.80                                 & 0.84                                & 0.00\%                                                               \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &                  MIRROR LOOK [CL ``swipe hair"] (\p{3})                                                & 1                                   & 4                                   & 2.50                                 & 1.05                                & 72.22\%                                                             \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{10}                                    & \multirow{-2}{*}{\parbox[t]{\lyriccolumnwidth}{Ooh, when I look in\newline{}the mirror}}         & PSE                                                     &                                       ME LOOK MIRROR (\p{6})                           & 3                                   & 7                                   & 5.20                                 & 1.79                                & 80.38\%                                                              \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &        [``hands on heart"] MELT ATTRACT (\p{2})                                                          & 2                                   & 9                                   & 4.33                                 & 2.50                                & 40.00\%                                                             \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{11}                                    & \multirow{-2}{*}{\parbox[t]{\lyriccolumnwidth}{I'll melt your heart\newline{}into two}}          & PSE                                                     &                                DISSOLVE YOUR HEART (\p{6})                                  & 3                                   & 4                                   & 3.80                                 & 0.45                                & 37.50\%                                                             \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &               ME LIKE FAMOUS PERSON [CL ``shine"]\newline{}[(2h) ``people looking"] (\p{3})                                                   & 2                                   & 7                                   & 3.67                                 & 1.86                                & 29.44\%                                                             \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{12}                                    & \multirow{-2}{*}{\parbox[t]{\lyriccolumnwidth}{I got that superstar\newline{}glow so}}           & PSE                                                     &                                   ME FAMOUS GLOW (\p{4}, \p{11})                               & 3                                   & 5                                   & 3.80                                 & 0.84                                & 25.83\%                                                             \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &           WE TWO DANCE (\p{12})                                                       & 1                                   & 3                                   & 2.33                                 & 0.82                                & 63.33\%                                                             \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{13}                                    & \multirow{-2}{*}{Do the boogie like}                     & PSE                                                     &                 DANCE LIKE (\p{4}, \p{8}, \p{11})                                                 & 2                                   & 3                                   & 2.20                                 & 0.45                                & 45.00\%                                                              \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &            [(2h) BPCL:1 ``MOVING SIDEWALK"]\newline{}FOLLOW MY BEAT (\p{2})                                                      & 1                                   & 7                                   & 4.17                                 & 2.14                                & 47.22\%                                                             \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{14}                                    & \multirow{-2}{*}{\parbox[t]{\lyriccolumnwidth}{Side step, right,\newline{}left to my beat}}      & PSE                                                     &                                      GLIDE LEFT RIGHT (\p{7})                            & 1                                   & 7                                   & 4.60                                 & 2.51                                & 20.71\%                                                             \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &               LIKE MOON JOIN ME SWEETHEART (\p{12})                                                   & 4                                   & 7                                   & 5.33                                 & 1.03                                & 41.00\%                                                             \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{15}                                    & \multirow{-2}{*}{\parbox[t]{\lyriccolumnwidth}{High like the moon,\newline{}rock with me, baby}} & PSE                                                     &                          HIGH LIKE MOON DANCE WITH ME (\p{6})                                        & 5                                   & 7                                   & 6.20                                 & 0.84                                & 59.38\%                                                             \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &             ME SEXY HOT (\p{12})                                                     & 2                                   & 4                                   & 3.00                                 & 0.89                                & 18.89\%                                                             \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{16}                                    & \multirow{-2}{*}{Know that I got that heat}              & PSE                                                     &                   KNOW ME HAVE HEAT (\p{8})                                               & 4                                   & 6                                   & 4.60                                 & 0.89                                & 42.00\%                                                              \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &            DEMONSTRATE TALK [``shake head"] (\p{10})                                                      & 2                                   & 7                                   & 5.00                                 & 1.67                                & 35.33\%                                                              \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{17}                                    & \multirow{-2}{*}{\parbox[t]{\lyriccolumnwidth}{Let me show you 'cause\newline{}talk is cheap}}   & PSE                                                     &                                  NO TALK JUST ACTION (\p{7})                                & 4                                   & 7                                   & 5.60                                 & 1.52                                & 29.88\%                                                             \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &          MY RHYTHM VIBRATE FOOT \newline{}["move right"]["move left"] (\p{3})                                                        & 1                                   & 6                                   & 3.67                                 & 1.63                                & 27.22\%                                                             \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{18}                                    & \multirow{-2}{*}{\parbox[t]{\lyriccolumnwidth}{Side step, right,\newline{}left to my beat}}      & PSE                                                     &                                  SIDE STEP RIGHT LEFT MATCH MY RHYTHM! (\p{11})                                & 4                                   & 7                                   & 6.00                                 & 1.41                                & 46.29\%                                                             \\\arrayrulecolor{lightgray}\hline
                                                        &                                                          & ASL                                                     &                   UNDERSTAND GO-AHEAD DANCE (\p{2})                                               & 1                                   & 4                                   & 2.67                                 & 1.03                                & 32.22\%                                                             \\\arrayrulecolor{tablegrayline}\cline{3-9}
\multirow{-2}{*}{19}                                    & \multirow{-2}{*}{Get it, let it roll}                    & PSE                                                     &               LET'S GO (\p{6})                                                   & 2                                   & 4                                   & 3.20                                 & 0.84                                & 18.33\%                      \\
\arrayrulecolor{black}\hline
\end{tabular}
\end{table}
